Causal Domain Restriction for Eikonal Equations

Many applications require efficient methods for solving continuous shortest path problems. Such paths can be viewed as characteristics of static Hamilton-Jacobi equations. Several fast numerical algorithms have been developed to solve such equations on the whole domain. In this paper we consider a somewhat different problem, where the solution is needed at one specific point, so we restrict the computations to a neighborhood of the characteristic. We explain how heuristic under/over-estimate functions can be used to obtain a causal domain restriction, significantly decreasing the computational work without sacrificing convergence under mesh refinement. The discussed techniques are inspired by an alternative version of the classical A* algorithm on graphs. We illustrate the advantages of our approach on continuous isotropic examples in 2D and 3D. We compare its efficiency and accuracy to previous domain restriction techniques. We also analyze the behavior of errors under the grid refinement and show how Lagrangian (Pontryagin's Maximum Principle-based) computations can be used to enhance our method.

==> figs/sat_oracle_vary_lambda.tex <==

\begin{figure}[H]
\begin{center}
\begin{adjustwidth}{-1.75cm}{}
\tabcolsep=0.05cm
\begin{tabular}{c c c c c c c}% c}
&
\multicolumn{6}{c}{\bf Satellite image solution, produced by FMM with A*} \\
% COMMENT REMOVED
&
{\em$\mathit{\lambda = 0}$\%} &
{\em$\mathit{\lambda = 30}$\%} & 
{\em$\mathit{\lambda = 70}$\%} &
{\em$\mathit{\lambda = 90}$\%} &
{\em$\mathit{\lambda = 95}$\%} &
{\em$\mathit{\lambda = 100}$\%} \\
&
\includegraphics[scale=\sinPicScale]{img/sat_oracle_contours/aa_00percent.pdf} &
\includegraphics[scale=\sinPicScale]{img/sat_oracle_contours/aa_30percent.pdf} &
\includegraphics[scale=\sinPicScale]{img/sat_oracle_contours/aa_70percent.pdf} &
\includegraphics[scale=\sinPicScale]{img/sat_oracle_contours/aa_90percent.pdf} &
\includegraphics[scale=\sinPicScale]{img/sat_oracle_contours/aa_95percent.pdf} &
\includegraphics[scale=\sinPicScale]{img/sat_oracle_contours/aa_100percent.pdf} %&
% COMMENT REMOVED
 \\ [-1ex]
\bf SA*: &
\footnotesize$p=0.823$, $\mathcal{E}^*_N=0$ &
\footnotesize$p=0.637$, $\mathcal{E}^*_N=0.0002$ &
\footnotesize$p=0.369$, $\mathcal{E}^*_N=0.009$ &
\footnotesize$p=0.200$, $\mathcal{E}^*_N=0.024$ &
\footnotesize$p=0.105$, $\mathcal{E}^*_N=0.026$ &
\footnotesize$p=0.046$, $\mathcal{E}^*_N=0.030$ \\
\bf AA*: &
\footnotesize $p=0.823$, $\mathcal{E}^*_N=0$ &
\footnotesize $p=0.657$, $\mathcal{E}^*_N=0$ &
\footnotesize $p=0.395$, $\mathcal{E}^*_N=0$ &
\footnotesize $p=0.213$, $\mathcal{E}^*_N=0$ &
\footnotesize $p=0.126$, $\mathcal{E}^*_N=0$ &
\footnotesize $p=0.051$, $\mathcal{E}^*_N\approx 10^{-9}$
\vspace{0.15cm} \\
&
\multicolumn{6}{c}{\includegraphics[scale=0.7]{img/sat_oracle_contours/colorbar.pdf}}
\end{tabular}
\end{adjustwidth}
\vspace{-.35cm}
\caption{\footnotesize Numerical results of FMM using A* techniques (we show the solution produced using AA* as it is qualitatively the same produced using SA*). We show the percent of domain computed $p$ and the relative error $\mathcal{E}^*_N$.}
\end{center}
\end{figure}

